Materialistic: Selecting Similar Materials in Images

Separating an image into meaningful underlying components is a crucial first step for both editing and understanding images. We present a method capable of selecting the regions of a photograph exhibiting the same material as an artist-chosen area. Our proposed approach is robust to shading, specular highlights, and cast shadows, enabling selection in real images. As we do not rely on semantic segmentation (different woods or metal should not be selected together), we formulate the problem as a similarity-based grouping problem based on a user-provided image location. In particular, we propose to leverage the unsupervised DINO features coupled with a proposed Cross-Similarity module and an MLP head to extract material similarities in an image. We train our model on a new synthetic image dataset, that we release. We show that our method generalizes well to real-world images. We carefully analyze our model's behavior on varying material properties and lighting. Additionally, we evaluate it against a hand-annotated benchmark of 50 real photographs. We further demonstrate our model on a set of applications, including material editing, in-video selection, and retrieval of object photographs with similar materials.

==> figures/layout/albedo_analysis.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/source/albedo_analysis}
    \caption{\textbf{Material selection with variation in albedo.} To analyze the behavior of the model with respect to changing albedo, we change the hue and saturation value on a diffuse sphere. The hue is sampled in range $[0, 2\pi]$ and saturation is sampled in $[0, 1]$. We select the central pixel on a grid of spheres with varying albedo. The scores are thresholded at 0.5 which results in selections of regions in spheres with neighboring albedo. Only the central sphere is selected with a threshold of 0.9 and more spheres are gradually selected as the threshold is lowered.
    
    \label{fig:albedo_analysis}
\end{figure}


==> old sections/0_introduction.tex <==
\section{Introduction}
% High-level motivation
The intensity and color of the light reaching a camera's pixels is a function of the material, lights, and geometry of the objects in the scene.
%
The human vision is capable of identifying all image regions that have the same material, irrespective of geometric and lighting variations. 
%
For example, we can identify that both chairs and the table in Fig~\ref{fig:overview} are made of the same material.
%
In this paper, our goal is to build a system that, given a query material (a selection of pixels), can automatically select all the image made of the same material.

% What can existing tools do?
Existing selections tools do not "understand" scene materials, and would therefore fail for our use case.
%
The lasso tool in Photoshop, for example, can only select neighboring pixels with similar RGB values.
%
The "object selection" tool can select whole objects, such as the chair in Fig~\ref{fig:overview}, but not entire materials across the scene.
%
At present, no existing tool can select all image regions with the same material.

Our method learns to perform this task by computing per-pixel embeddings for the input image, and computing the cosine distance between the embedding of the selected pixel and embedding of all other pixels.
%
It is trained with a supervised contrastive loss.
%
At test time, given a single image and a few pixel selection on the image by the user, our method generates a map of pixels that have the same material.
%
The user can further tweak the predicted selection by tweaking a sensitivity threshold.
%
Choosing a higher threshold further restricts the selection based on the similarity score.
%
Our system is trained on a synthetic dataset of randomized geometric primitives with procedurally generated materials from Substance 3D, which are rendered in a indoor scene setup.
%
Despite being trained on synthetic data, our model shows promising generalization to real photographs. 

This technology can have significant impact across Adobe products. Adding to the palette of selection tools available to our users, and enabling novel editing tasks like material replacement in photographs, or complex downstream analysis technologies, such as improving scene understanding, enabling automatic material and BRDF extraction from a single image.

\input{figures/layout/overview}


% Current state of the project
While our current model only uses the RGB input as input along with material label based contrastive loss for training, we aim to further improve it by:
\begin{enumerate}
    \item adding lighting and geometric cues (such as depth, normal) to our model inputs, and
    \item making the model more robust by further finetuning on more realistic indoor renderings from the HyperSim dataset\cite{hypersim}.
\end{enumerate}


==> old sections/1_dataset.tex <==
\section{Dataset}
We render a dataset of indoor scenes using Blender where we spawn 5--15 primitive objects (from cubes, cones, cylinders, spheres, torus) in the scene. Each of these objects has a random size: each of the physical parameters, such as height, radius, side length, are sampled from a predefined uniform distribution.
%
We assign each object a random material, sampled from a collection of 16858 procedurally materials, procedurally generated using Substance 3D.
%
The scene is lit using 1--5 light sources, where each light source is an area lamp with intensity uniformly sampled from $[200, 600]$ watts, and an area of 0.5--4 square meters.
%
Our dataset contains 25000 training samples, where each sample is a 16-bit rendering.
%
During training, we augment our training set by applying random white balance, exposure correction, gamma correction, and JPEG compression to add variations and make our model better able to generalize to a wide variety of real-world inputs.
%
Furthermore, we apply spatial image transformations such as random horizontal flip and random crops to the input during training. 

==> old sections/2_method.tex <==
\section{Method}
Given an input image, we first compute a learned feature embedding using a 2D UNet~\cite{ronneberger2015u}.
%
These per-pixel embedding act as the image representation on top of which we compute the cosine distance from one pixel to all the other pixels, which gives us a measure of how close their material properties are.
%
During training, we train the model using a contrastive loss, encouraging the feature embedding of pixels labeled with the same material identifier to be close, and pushing aparts the feature embeddings of pixel with distinct materials.
%
This contrastive loss is computed using the ground truth material labels, which we compute when rendering the scene in Blender.

\subsection{Supervised contrastive loss to train the embedding}

We learn the sample embeddings by optimizing a contrastive loss, with known material labels.
%
Specifically, we sample $P$ positive and $N$ negative samples from the set of pixel embeddings for the image.
%
For a given anchor pixel, positive samples are pixels that have the same material labeled in the ground truth. Negative samples have different labels. The contrastive loss is computed as 

\begin{equation}
    \textit{Loss}_{Contrastive}(x_i) = - \log \frac{\sum_{x_j \in P} e^{\textit{sim}(x_i, x_j)/\tau}}{\sum_{x_j \in P} e^{\textit{sim}(x_i, x_j)/\tau} + \sum_{x_j \in N} e^{\textit{sim}(x_i, x_j)/\tau}},
\end{equation}

where $\textit{sim}(x_i, x_j) = \frac{x_i \cdot x_j}{ \max\left(||x_i|| ||x_j||, \epsilon\right)}$,$\tau$ is a temperature that controls the sharpness of the affinity, $x_i$ is the embedding for pixel $i$, and $P$ and $N$ are the numbers of randomly selected positive and negative samples. 

\subsection{Test-time selection prediction}
% How is the model inferred? Multiple selection? Multiple negative selection?
At test time, we compute the embeddings for each pixel of the image using the trained UNet.
%
Then for the pixel selected by the user (the anchor), we compute the cosine similarity between its embedding and those of all the other pixels. 
%
This yields a similarity map with values in $[-1, 1]$ describe how similar each pixel's material is to the anchor.
%
We then threshold the similarity scores to obtain a mask corresponding to the selected region, in which the material appearance is similar.
%
The threshold can be adjusted by the user to refine the selection.
%
Increasing the threshold reduces the predicted region.

\subsection{User interface for material selection}
%
Furthermore, we enable the selection of multiple anchor points to improve the selected region as shown in Fig.~\ref{fig:demo}, by providing additional positive examples of the material.
%
We compute the cosine similarity of all points with respect to the selected points, and compute the similarity score for a pixel to be the maximum of the similarity scores computed for each point selected.
%
We again apply a threshold to the result.

Note that in our current implemention, additional selections can only expand the selected region, but a similar approach can be used to shrink the selected region: if we also allow the user to choose points from materials that do not correspond to the material they wish to select, we can substract the region computed from the additional negative points from the selection. 

\input{figures/layout/demo}

==> old sections/3_results.tex <==
\section{Results}

\input{figures/layout/synthetic_results}
% Results on synthetic
In Fig.~\ref{fig:synth_results}, we present results on the synthetic samples where the image is rendered in Blender with primitive objects. 

\input{figures/layout/real_results}

% Results on real
We show the performance of our model on real images of indoor and outdoor scenes in Fig.~\ref{fig:real_results}. 


==> old sections/4_conclusion.tex <==
\section{Conclusion}

% Why is this important? Impact on Adobe products, graphics, vision, robotics
Our technology uses a convolutional neural network trained using a supervised contrastive loss to learn an image representation that enables user guided material selection.
%
This provides an automatic solution to material-based selections than existing tools, such as lasso selection and object selection, cannot achieve.
%
The ability to select image regions based on material is important for downstream applications at Adobe.
%
It enables material acquisition, material swapping from a single image, material-based image processing, for instance.
%
This technology can also be a useful cue for denoising and super-resolution methods.
%
Moreover, our representation is useful for scene understanding, since it provides a strong prior for segmentation and object representation impacting vision and robotics applications.

% What are the next steps?
Our current prototype achieves good results on both synthetic and real scenes.
%
We aim to further improve its robustness and generalization to real world images by incorporating geometric information such as depth and normal, and lighting information. 
